Metacat: a categorical framework for formal systems

We present a categorical framework for formal systems in which inference rules with $m$ metavariables over a category of syntax $\mathscr{S}$, taken to be a cartesian PROP, are represented by operations of arity $k \to n$ equipped with spans $k \leftarrow m \to n$ in $\mathscr{S}$, encoding the hypotheses and conclusions in a common metavariable context. Composition is by substitution of metavariables, which is the sole primitive operation, as in Metamath. Proofs in this setting form a symmetric monoidal category whose monoidal structure encodes the combination and reuse of hypotheses. This structure admits a proof-checking algorithm; we provide an open-source implementation together with a surface syntax for defining formal systems. As a demonstration, we encode the formulae and inference rules of first-order logic in Metacat, and give axioms and representative derivations as examples.

==> Makefile <==
OUT := build
DOCS := main
SVG_PDFS := $(patsubst %.svg,%.pdf,$(wildcard *.svg))

BUILD_CMD := pdflatex -interaction=nonstopmode -output-directory $(OUT)

all: pdf

$(OUT):
	mkdir -p $(OUT)

pdf: main

main: $(OUT)/main.pdf

$(OUT)/%.pdf: %.tex bib $(SVG_PDFS) | $(OUT)
	$(BUILD_CMD) $<
	if [ -f $(OUT)/$*.aux ]; then \
		set -e; cd $(OUT); BIBINPUTS=..: BSTINPUTS=..: bibtex $*; \
	fi
	$(BUILD_CMD) $<
	$(BUILD_CMD) $<

%.pdf: %.svg
	inkscape $< --export-type=pdf --export-filename=$@

bib: *.bib
	cat *.bib > $(OUT)/main.bib

view:
	zathura build/main.pdf &

